Predicting integers from continuous parameters

We study the problem of predicting numeric labels that are constrained to the integers or to a subrange of the integers. For example, the number of up-votes on social media posts, or the number of bicycles available at a public rental station. While it is possible to model these as continuous values, and to apply traditional regression, this approach changes the underlying distribution on the labels from discrete to continuous. Discrete distributions have certain benefits, which leads us to the question whether such integer labels can be modeled directly by a discrete distribution, whose parameters are predicted from the features of a given instance. Moreover, we focus on the use case of output distributions of neural networks, which adds the requirement that the parameters of the distribution be continuous so that backpropagation and gradient descent may be used to learn the weights of the network. We investigate several options for such distributions, some existing and some novel, and test them on a range of tasks, including tabular learning, sequential prediction and image generation. We find that overall the best performance comes from two distributions: Bitwise, which represents the target integer in bits and places a Bernoulli distribution on each, and a discrete analogue of the Laplace distribution, which uses a distribution with exponentially decaying tails around a continuous mean.

==> bak/old_comments.tex <==
% ------------------ ------ ------------------ 
% ------------------ --RL-- ------------------ 
% ------------------ ------ ------------------ 
%The research shows the great potential of the Discrete Weibull distribution for regression tasks, especially in comparison with the Poisson distribution for regression \cite{cameron2013regression}. Kalktawi et al. \cite{kalktawi2015simple} stands out as a significant contribution, bridging a gap in the existing methodology of the Discrete Weibull Distribution. Kalktawi introduces a versatile and computationally efficient approach to address the common challenges in count data modeling, particularly dispersion and the presence of excessive zeros. The application of their model to diverse real-world datasets underscores its practical relevance and potential to significantly improve the analysis of count data in various fields, setting a new precedent for future research and application in discrete data analysis.


%similarly to what we are doing in our paper btw.
%Similar to Contin, Tovissodé et al. \cite{math9050555} covers balanced discretization for modeling count data, specifically addressing the challenges encountered in regression analysis due to various levels of data dispersion equi-, under-, and over-dispersion. Balanced discretization offers a solution by discretizing continuous probability distributions in a way that expectations are preserved, enabling the exact inference for count data across all dispersion levels. The core contribution of this work is the introduction of the balanced discrete gamma distribution, a family of distributions that can accurately model count data with different dispersion levels. This method simplifies the generation of pseudo-random variate through a probabilistic rounding mechanism, making it especially suitable for count regression models where data do not adhere to the strict equi-dispersion assumption of the Poisson model. The only disadvantage of this implementation is the limitations in calculating the backward gradient for these distributions, which CONTIN in contrast can do.



% ------------------ ------ ------------------ 
% ------------------ Experiments ------------------
% ------------------ ------ ------------------ 
% Below are notes that need to still be added in text: \\
% All experiments are done with the random seed set to 42. \\
% Talk about the activations of the distributions (CONTIN, Dnormal and Dweib)

% %Need to move this elsewhere

% Each experiment is executed with a sweep over the learning rates: 3.4e-3, 1e-3, 3.4e-4, 1e-4, 3.4e-5 and 1e-5. The best performing hyperparameter is used for the test set.
% \\\\

%The experiments aim to demonstrate the flexibility of the proposed distribution functions in handling count data, as opposed to standard continuous methods like squared error loss, which may fail to capture the discrete nature of the target variable. 

% By conducting these experiments, we aim to validate the hypothesis that distribution-specific modeling improves the prediction accuracy and generalizability of models in scenarios where the target variable is inherently discrete.  


%During training, validation and testing, the loss averaged over the number of instances.

% As shown in Figure \ref{fig:target_variance}, the Upvotes dataset presents a greater challenge for modeling due to the higher variance in target values compared to the Bicycles dataset.

% Compared to the categorical distribution, these would model the ordinal aspect of the output values inherently, and save memory in the size of the output layer, as attempted by \cite{salimans2017pixelcnnimprovingpixelcnndiscretized}. Compared to the continuous relaxations, they would provide a more interpretable value in bits for the log-loss, which could be combined better with discrete labels, like a description of the image in natural language.

% We consider this a preliminary investigation, using only simple datasets and one basic model, to see whether the choice of a discrete output distribution would be feasible in principle. A full investigation over more complex generative models (like diffusion models) and using more high-resolution datasets is left to future work. 


% TODO Are these the right citations? They seem too late (MNIST is from the 90s). Best version I can find is from 2012

% As a model, we use a Gated PixelCNN architecture \cite{oord2016conditionalimagegenerationpixelcnn}. This autoregressive generative model employs masked convolutions to enforce a causal ordering over pixels, ensuring each pixel is predicted based only on previously generated ones. Our implementation uses a two-stack architecture with vertical and horizontal convolutional streams connected via gated activations, enabling the model to capture long-range spatial dependencies while maintaining the autoregressive property. We incorporate coordinate conditioning (CoordConv) to provide explicit positional information to the network.

% For the MNIST and FashionMNIST datasets, the model only trains and generates a single grayscale pixel, only 1 feature. The CIFAR10 dataset has RGB channels and therefore the model predicts 3 pixels / features, one for red, one for green and one for the blue channel. Per channel and per pixel a distribution function is created for predicting the pixel value.


% Dnormal
%As the problem of modeling discrete count data under a distribution, the normal distribution is a quite obvious choice. The model has continuous parameters and continuous outputs, where the latter can be made discrete. by rounding the output of the distribution. We use the standard definition of the CDF of the normal distribution as equation \ref{eq:dnormal_cdf} with the addition of $\epsilon$ for stabilization. The Erf function is defined as in equation
%\ref{eq:erf_func}. 
%
%To calculate the log probability, we determine the probability mass assigned to each integer \( x \) as the difference in the cumulative distribution function (CDF) between \( x \) and \( x+1 \). This ensures that the probability for each discrete value corresponds to the area under the normal curve between two consecutive integers. The log probability is then computed as seen in equation \ref{eq:logprob_dnormal}.
%\begin{equation}
%    \log P(x) = \log(\Phi(x+1) + \epsilon - \Phi(x))
%    \label{eq:logprob_dnormal}
%\end{equation}

%\textbf{Requires still some why}


% ------------------ ------ ------------------ 
% ------------------ Contin ------------------ 
% ------------------ ------ ------------------ 

% % When the dispersion parameter $\gamma$ is 0 all the probability is concentrated on $\lfloor\mu\rfloor$ and $\lceil\mu\rceil$. As $\gamma$ increases, the probability mass of these values decreases and the distribution spreads more across the surrounding integers.
% % To calculate the probabilities for the remaining discrete values in the distribution, separate geometric series are employed for the left and right tails. The left tail begins with the probability assigned to $\lfloor\mu\rfloor$, while the right tail starts with the probability assigned to $\lceil\mu\rceil$.

% Equation \ref{eq:logprob calculation} provides the log probability mass function (PMF) that is shared among the different forms, calculating the logarithmic probability of observing the value x, given parameters $\mu$ and $\gamma$. Equation \ref{eq:contin_unbounded} shows the unbounded PMF function, equation \ref{eq:contin_oneway} shows the one-way bounded PMF function, and equation \ref{eq:contin_twoway} the two-way bounded PMF function. To further illustrate CONTIN Fig. \ref{fig:mu_balanced} provides a clear illustration of the discretization of the $\mu$ value.

% \begin{adjustbox}{center}
%     \begin{equation}
%         \begin{aligned}
%             x &= \text{target value} \\
%             b_p &= \begin{cases}
%                 b_f & \text{if } x \leq \mu \\
%                 b_c & \text{else } x > \mu
%             \end{cases} \\
%             d &= \begin{cases}
%                 \lfloor\mu\rfloor-x & \text{if }  x \leq \mu \\
%                 x-\lceil\mu\rceil & \text{else } x > \mu
%             \end{cases} \\
%             \log P(X = x | \mu, \gamma) &= \log{(b_p)}+d\cdot\log(\gamma) \\
%         \end{aligned}
%         \label{eq:logprob calculation}
%     \end{equation}
% \end{adjustbox}

% \vspace{1cm}

% \begin{adjustbox}{center}
%     \begin{equation}
%         \begin{aligned}
%             \log P(X = x | \mu, \gamma) &=  \log{(1-\gamma)} - \log{(1+\gamma)} + \log P(X = x | \mu, \gamma)
%         \end{aligned}
%         \label{eq:contin_unbounded}
%     \end{equation}
% \end{adjustbox}
% \vspace{1cm}
% \begin{adjustbox}{center}
%     \begin{equation}
%         \begin{aligned}
%             x &= \text{target value} \\
%             x &= \begin{cases}
%                 x - \text{bound} & \text{if lower bounded} \\
%                 -(x - \text{bound}) & \text{else upper bounded}
%             \end{cases} \\
%             \mu &= \begin{cases}
%                 \mu - \text{bound} & \text{if lower bounded} \\
%                 -(\mu - \text{bound}) & \text{else upper bounded}
%             \end{cases} \\
%             \log P(X = x | \mu, \gamma) &= \log{(1-\gamma)}-\log(b_f\cdot(1-\gamma^{\lfloor\mu\rfloor+1})+b_c)+\log P(X = x | \mu, \gamma)
%         \end{aligned}
%         \label{eq:contin_oneway}
%     \end{equation}
% \end{adjustbox}
% \vspace{1cm}
% \begin{adjustbox}{center}
%     \begin{equation}
%         \begin{aligned}
%             \gamma_{l} & = b_f\cdot(1-\gamma^{\lfloor\mu\rfloor-\text{lower bound}+1})\\
%             \gamma_{u} & = b_c\cdot(1-\gamma^{\text{upper bound} - \lceil\mu\rceil + 1})\\
%             \log P(X = x | \mu, \gamma) &= \log{(1-\gamma)} - \log(\gamma_{l}+\gamma_{u})+\log P(X = x | \mu, \gamma)
%         \end{aligned}
%         \label{eq:contin_twoway}
%     \end{equation}
% \end{adjustbox}

% \begin{figure}[!hbt]
%     \centering
%     \begin{adjustbox}{center}
%         \includegraphics[width=1.3\linewidth]{balanced_mu.png}
%     \end{adjustbox}
%     \caption{Visual example of the convex combination of $\mu$.}
%     \label{fig:mu_balanced}
% \end{figure} 


% ------------------ ------ ------------------ 
% ------------------ Conclusion ------------------ 
% ------------------ ------ ------------------ 
% -- Discrete distributions can be competitive with continuous relaxations, although continuous relaxations still offer best performance in all datasets tested.
% -- Therefore, discrete distributions are a good option \emph{if} continuous relaxations are undesirable for some reason, for example, because a loss in bits is required. 
% -- We note that performance in bits is well correlated with RMSE, but not always perfectly so. It depends on the task which metric should be considered leading. 
% -- However, discretizations of a well-performing continuous relaxation do not perform as well as other alternatives. 
% -- In preliminary experiments in generative modeling, we see some promising results 

% -- Bitwise is very sensitive to insecurity when it comes to higher bits, if those are not certain the entire prediction will be off by many (and cause very high variance).

% \subsection{Limitations and future work}

% -- 
% In addition, future work would analyse the capabilties of replacing the requirement for categorical output distributions of LLMs with a discrete distributed model. This would in turn reduce the number of output nodes required to make predictions over the vocabulary size.
% -- Removed: not sure this would make sense, since the token space is not ordinal. Maybe in some domains?


% ------------------ ------ ------------------ 
% ------------------ Bitwise ------------------ 
% ------------------ ------ ------------------ 
%Then, let \[
%S_k(\bpi) = \sum_{\x \in \mB^k} \bpi^{\x}\p 
%\]
%
%Now, note that 
%\begin{lemma}
%$S_k(\bpi) = 1$ for any $k$ and any $\bpi$
%\end{lemma}
%\begin{proof} We show this by induction. First, $S_1 = \pi_1 + \pi_1^\ndot = 1$.
%Then, 
%\begin{align*}
%S_k(\bpi) &= \sum_{\x \in \mB^k} \pi_1^{\x} \times \ldots \times \pi_k^{\x}  \\ 
%&= \pi_1 \sum_{\x \in \mB^{k-1}} \pi_2^{\x} \times \ldots \times \pi_k^{\x} + \pi_1^\ndot \sum_{\x \in \mB^{k-1}} \pi_2^{\x} \times \ldots \times \pi_k^{\x}\\
%&= (\pi_1 + \pi_1 ^\ndot)S_{k-1}(\bpi_{2:}) = 1 \p 
%\end{align*}
%Where $S_{k-1}(\cdot) = 1$ follows from the induction hypothesis.
%\qed
%\end{proof}



%Finally, we introduce Bitwise, a way of representing discrete numbers as a multi-binary classification problem. This method is not new, but is not widely applied to the problem of modeling count data. With Bitwise, integer numbers are transformed into unsigned binary bit-strings, where the numbers of bits (up to n) determine the maximum representable integer. While this imposes a two-way boundary, increasing the bit count significantly raises the upper limit. The representation is flexible enough to accommodate different encodings to allow for different boundary limitations, for example encoding negative numbers through two's complement encoding.
%
%For this study, we focus on a 32-bit unsigned binary encoding as well as encoding using two's complement for negative ranges. 32 bit positions gives leaves enough room for target ranges to be both, positive and negative as well as to be large integer values. 
%
%To assess model performance, we employ Bitwise Binary Cross Entropy (BBCE). This loss function compares the model's output bit-string to the target integer value (which is also encoded in bit-string form). Before the model's output bit-string is computed in BBCE it is first activated using Log Sigmoid, similarly to regular activation for Binary Cross Entropy with Logits. To reduce noise in the predictions of models the bits are weighted depending on its order, since a mistake in a higher order bit shifts the number significantly more than a mistake in a lower order bit. This weighting method is done by calculating multiplying the BBCE with a number range of order $2^n$. The final loss per bit is then summed and averaged over the batch dimension. 
%
%\subsection{Bitwise Mean and Variance}
%In equation \ref{eq:mean_bitwise} the calculation of the mean of Bitwise can be found. <- I think this should maybe be moved to the appendix now that we have the CONTIN explanation above.
%\begin{equation}
%\begin{aligned}
%    p_\theta &= \{\theta_1 ... \theta_n\} \\
%    X &= \{2^0 ... 2^n\} \\
%    P(X=x) &= p_\theta \\
%    E(X) &= \mu = \sum_{i=0}^{n} x_i \cdot P(x_i) \\
%    E_{bnp} &= \sum_{i=0}^{n} b_i \cdot \theta_i \\
%    \mu &= \sum_{i=0}^{n} 2^i \cdot \theta_i
%\end{aligned}
%\label{eq:mean_bitwise}
%\end{equation}
%
%In equation \ref{eq:var_bitwise} the calculation of the variance of Bitwise can be found. <- I think this should maybe be moved to the appendix now that we have the CONTIN explenation above.
%\begin{equation}
%\begin{aligned}
%    p_\theta &= \{\theta_1 ... \theta_n\} \\
%    X &= \{2^0 ... 2^n\} \\
%    P(X=x) &= p_\theta \\
%    Var(X) &= E[X^2] - (E[X])^2 \\
%    E[X^2] &= \sum_{i=0}^{n} b_i^2 \cdot \theta_i \\
%    Var(X) &= \sum_{i=0}^{n} b_i^2 \cdot \theta_i - (\sum_{i=0}^{n} b_i \cdot \theta_i)^2 \\
%    Var(X) &= E[(X-\mu)^2] = \sum_{i=0}^{n} b_i^2 \cdot \theta_i - (\sum_{i=0}^{n} b_i \cdot \theta_i)^2 \\
%    Var(X) &= E[(X-\mu)^2] = \sum_{i=0}^{n} (2^i - \mu)^2 \cdot \theta_i
%\end{aligned}
%\label{eq:var_bitwise}
%\end{equation}



==> bak/old_results.tex <==
\subsection{Count Data Regression}
We evaluated several loss functions for count data regression tasks on four distinct datasets: Bicycles, Upvotes, Migration, and Maestro. Performance was assessed using two primary metrics presented in Table \ref{tab:test_res}: Bits, which reflects the model's negative log-likelihood (base 2) and serves as a proxy for compression efficiency or goodness-of-fit from a likelihood perspective (lower is better), and Root Mean Squared Error (RMSE), which measures the accuracy of the predicted mean count value against the true counts (lower is better). The \texttt{MSE} loss, by definition, optimizes directly for squared error and thus does not have a comparable Bits score ('na' in the table). The \texttt{Dweib} model failed to produce results for the Migration dataset ('na').

Analyzing the Bits metric reveals that the \texttt{Bitwise} loss function generally provides the best likelihood fit for most datasets. It achieved the lowest Bits scores on Bicycles (\textbf{9.22}), Upvotes (\textbf{6.86}), and Maestro (\textbf{5.65}). This suggests that its underlying assumptions (likely related to discrete probability distributions) align well with the data structure in these cases. However, on the Migration dataset, \texttt{CONTIN} achieved the best Bits score (\textbf{21.78}), indicating it provided a better likelihood fit for that specific, potentially more complex, data distribution compared to \texttt{Bitwise} (27.05) and \texttt{Dnormal} (26.16). \texttt{Dnormal} showed moderate performance, generally higher than \texttt{Bitwise} but comparable to \texttt{CONTIN} in some cases (e.g., Maestro). \texttt{Dweib} consistently performed poorly in terms of Bits where results were available, particularly on the Upvotes dataset (109.20), suggesting its distributional assumptions are a poor match for these count data tasks.

A distinctly different pattern emerges when evaluating prediction accuracy via RMSE. The \texttt{MSE} loss function, which directly minimizes squared error, consistently delivered the lowest RMSE across all four datasets: Bicycles (\textbf{44.80}), Upvotes (\textbf{658.59}), Migration (\textbf{65075.51}), and Maestro (\textbf{43.39}). This highlights its effectiveness when the primary goal is accurate prediction of the mean count.

Among the other methods, performance varied significantly. \texttt{Bitwise} achieved a competitive RMSE only on the Maestro dataset (44.39), very close to \texttt{MSE}. However, its RMSE was considerably higher on Bicycles (156.67) and Upvotes (751.81), and extraordinarily high on the Migration dataset (approx. $3.5 \times 10^9$), indicating poor predictive accuracy in these cases despite good Bits scores. \texttt{CONTIN} and \texttt{Dnormal} generally exhibited higher RMSE values than \texttt{MSE}, suggesting lower prediction accuracy. Their performance was roughly comparable on Bicycles and Maestro. On Upvotes, \texttt{Dnormal} (1826.73) was better than \texttt{CONTIN} (2425.13). Notably, on the challenging Migration dataset, both had very high RMSEs, but \texttt{Dnormal}'s (\textbf{175805.53}) was slightly lower than \texttt{CONTIN}'s (175810.58), though both were significantly outperformed by \texttt{MSE}. \texttt{Dweib} consistently showed poor predictive performance with high RMSE values where available.

The results highlight a clear trade-off between optimizing for likelihood (Bits) and prediction accuracy (RMSE) in count data regression. \texttt{Bitwise} excels in providing a good likelihood fit (low Bits) for several datasets but often struggles with accurate mean prediction (high RMSE), especially on challenging datasets like Migration. Conversely, \texttt{MSE} is the undisputed leader for prediction accuracy (lowest RMSE) by design, but does not offer a comparable likelihood-based metric.

\texttt{CONTIN} and \texttt{Dnormal} represent intermediate approaches, with \texttt{CONTIN} achieving the best Bits score on Migration, and \texttt{Dnormal} showing slightly better RMSE than \texttt{CONTIN} on Upvotes and Migration (excluding \texttt{MSE}). However, neither consistently matched \texttt{Bitwise} on Bits nor \texttt{MSE} on RMSE. \texttt{Dweib} appears generally unsuitable for these datasets, underperforming significantly on both metrics and failing entirely on the Migration task. The extreme RMSE values observed for several methods on the Migration dataset underscore its difficulty, likely due to high variance, complex dependencies, or outliers not well-handled by standard count models other than direct \texttt{MSE} optimization.

\begin{table*}[hbt!]
  \centering
  \sisetup{detect-weight,
         group-minimum-digits = 4,
         mode=text    % for bold
         }
  \caption{Test set results bicycles, migration, upvotes and maestro, best in bold. Unbounded Dalap indicated with an *}
  \begin{adjustbox}{center}

      \begin{tabular}{ l  
      	S[table-format=2.2] S[table-format=3.2]   % bicycles
      	S[table-format=3.2] S[table-format=4.2]   % upvotes
      	S[table-format=3.2] S[table-format=10.2]  % migration
      	S[table-format=1.2] S[table-format=2.2]   % maestro
      	} 
      	\hline
        ~ & \multicolumn{2}{c}{Bicycles} & \multicolumn{2}{c}{Upvotes} &  \multicolumn{2}{c}{Migration} &  \multicolumn{2}{c}{MAESTRO} \\
        ~         & {Bits}      & {RMSE}       & {Bits}      & {RMSE}        & {Bits}       & {RMSE}          & {Bits}      & {RMSE} \\
        \Xhline{1pt}
        {Bitwise}          & 9.22        & 156.67       & \ubold 6.86 & 751.81        & 27.05        & 3502410016.00   & \ubold 5.65 & 44.39 \\
        {CONTIN}           & 15.34       & 206.39       & 9.84        & 2424.78       & 21.78        & 175810.57       & 7.11        & 45.81 \\
        {Dalap}            & \ubold 7.09*& 53.46        & 10.20       & 3304.26       & 25.60        & 175805.51       & 7.25        & 50.72 \\
        {Laplace}          & 16.49       & 207.34       & 9.28        & 2005.18       & 74.74        & 175805.52       & 6.82        & 45.02 \\
        {Dnormal}          & 16.07       & 209.65       & 9.25        & 1826.73       & 26.16        & 175805.53       & 7.11        & 45.76 \\
        {Dweib}            & 11.32       & 268.17       & 109.20      & 2190.83       & {na}         & {na}            & 7.22        & 45.59 \\
        {MSE}              & {na}        & \ubold 44.80 & {na}        & \ubold 658.59 & {na}         & \ubold 65075.51 & {na}        & \ubold 43.39 \\
        \hline
      \end{tabular}
  \end{adjustbox}
  \label{tab:test_res}
\end{table*}

\subsection{VAE Performance Evaluation}
\label{sec:vae_results} % Optional: Add a label for the subsection if you want to reference it

We evaluated the performance of Variational Autoencoders (VAEs) trained with various reconstruction loss functions on the MNIST, Fashion-MNIST (FASHION), and CIFAR10 datasets. Performance was measured in bits per dimension (bits) on the test set, where lower values indicate better generative modeling. The quantitative results are summarized in Table \ref{tab:test_vae}, and qualitative examples of reconstructions are presented in Figures \ref{fig:mnist_res}, \ref{fig:fashion_res}, and \ref{fig:cifar_res}.

The choice of reconstruction loss significantly impacts VAE performance, with optimal choices varying across datasets.
\begin{itemize}
    \item On \textbf{MNIST}, the \texttt{Contin} loss achieved the best performance with \textbf{11.43 bits}, closely followed by \texttt{Laplace} (14.80 bits) and \texttt{Bitwise} (14.94 bits). \texttt{Dnormal} (25.66 bits) performed less competitively, while \texttt{Dweib} yielded a very poor score (435.66 bits), suggesting its distributional assumptions are ill-suited for this dataset.
    \item On \textbf{Fashion-MNIST}, \texttt{Contin} again demonstrated the strongest performance (\textbf{30.81 bits}), with \texttt{Laplace} (31.18 bits) being highly competitive. \texttt{Bitwise} (37.72 bits) and \texttt{Dnormal} (42.29 bits) followed, while \texttt{Dweib} (59.08 bits) showed considerable improvement compared to MNIST but still lagged behind.
    \item On \textbf{CIFAR10}, the trend shifted. The \texttt{Laplace} loss achieved the best result (\textbf{206.64 bits}), slightly outperforming \texttt{Contin} (210.85 bits). \texttt{Dnormal} (230.73 bits) and \texttt{Bitwise}  were less effective, and \texttt{Dweib} (261.07 bits) was the weakest among the standard distributions.
\end{itemize}
Interestingly, the \texttt{BCE} (Binary Cross-Entropy) loss yielded negative bits values for MNIST (-28.01) and Fashion-MNIST (-15.43). While numerically the lowest, negative values in this context typically arise when the model assigns high probability (>0.5) to the correct pixel values (often assuming pixels are binary or Bernoulli distributed), leading to positive log-likelihood components in the calculation. This indicates high confidence in pixel-level predictions for these grayscale datasets but makes direct comparison difficult. Notably, \texttt{BCE} performed poorly on the color CIFAR10 dataset (15.63 bits relative to the significantly higher scores of other losses, but still much worse than Laplace/Contin on this dataset).

The visual results presented in Figures \ref{fig:mnist_res} (MNIST), \ref{fig:fashion_res} (FASHION), and \ref{fig:cifar_res} (CIFAR10) complement the quantitative findings. Each figure compares original images (left column within each loss panel) to VAE-generated reconstructions (right column).
\begin{itemize}
    \item For \textbf{MNIST} and \textbf{FASHION}, the reconstructions from \texttt{Contin}, \texttt{Laplace}, \texttt{Bitwise}, and \texttt{BCE} generally appear sharp and faithful to the originals, aligning with their strong quantitative scores. \texttt{Dnormal} reconstructions sometimes show slight blurring or artifacts (e.g., FASHION). \texttt{Dweib} reconstructions are visibly degraded, particularly on MNIST, exhibiting significant noise or distortion, consistent with its high bit scores.
    \item For \textbf{CIFAR10}, reconstructions across all loss functions exhibit noticeable blurriness, a common characteristic of VAEs applied to complex natural image datasets. However, visual differences corresponding to the quantitative results are still apparent. \texttt{Laplace} and \texttt{Contin}, the top quantitative performers, produce relatively clearer (though still blurry) reconstructions compared to \texttt{Dnormal}, \texttt{Bitwise}, and especially \texttt{Dweib}, which shows significant noise and color artifacts. The qualitative results reinforce the quantitative ranking on this more challenging dataset.
\end{itemize}

\noindent Overall, the \texttt{Contin} and \texttt{Laplace} loss functions demonstrate robust and often leading performance across the tested datasets, both quantitatively and qualitatively. The optimal choice can be dataset-dependent, with \texttt{Contin} favoured for MNIST/FASHION and \texttt{Laplace} for CIFAR10 in our experiments. Distributional assumptions like \texttt{Dnormal} and particularly \texttt{Dweib} proved less suitable for modeling these image datasets within a VAE framework. The \texttt{Bitwise} loss offers a reasonable baseline, while \texttt{BCE} shows high confidence on binary-like data but struggles comparatively on complex color images and presents interpretation challenges due to negative bit scores. The visual quality of reconstructions generally aligns well with the bit performance metrics.

\begin{table*}[hbt!]
  \centering
  \caption{Test set results in bits on MNIST, FASHION, and CIFAR10 (closer to zero is better, best in bold). * signifies batch normalization, ** unbounded.}
  \begin{adjustbox}{center}
    \begin{tabularx}{\textwidth}{ l | X | X | X }
      \hline
      Loss Type & \multicolumn{1}{l|}{MNIST} & \multicolumn{1}{l|}{FashionMNIST} & \multicolumn{1}{l}{CIFAR10} \\
      \Xhline{1pt}  
      Bitwise               & 15.20           & 37.33             & 249.13           \\
      % Contin                & \ubold 11.43    & 30.81             & 210.85         \\
      Dalap                 & \ubold 11.47*   & \ubold 29.70      & \ubold 205.72    \\
      Dnormal               & 21.41           & 33.21**           & 208.53**         \\
      Dweib                 & 56.09*          & 60.26             & 262.64           \\
      Laplace               & 12.92*          & 31.16             & 206.33           \\
      Continuous Bernoulli  & 1730.45*        & 1317.83           & 7733.37          \\
      Categorical           & 629.94          & 1776.42           & 12247.26         \\
    \end{tabularx}
  \end{adjustbox}
  \label{tab:test_vae}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{MNIST.png}
    \caption{Epoch 99 of MNIST dataset, target data on the left and generated data on the right.}
    \label{fig:mnist_res}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{FASHION.png}
    \caption{Epoch 99 of FASHION dataset, target data on the left and generated data on the right.}
    \label{fig:fashion_res}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{CIFAR10.png}
    \caption{Epoch 99 of CIFAR10 dataset, target data on the left and generated data on the right.}
    \label{fig:cifar_res}
\end{figure}

==> bak/results2.tex <==
\subsection{Count Data Regression}
We evaluate several distribution functions for integer-valued regression on four datasets: Bicycles, Upvotes, Migration, and Maestro. Performance is reported in Tables \ref{tab:test_res_non_mixed} and \ref{tab:test_res_mixture} using two metrics: Bits (negative log-likelihood in base 2; lower is better) and RMSE (accuracy of the predicted mean; lower is better). 

Dalap performs best across all datasets in bits, except for the bicycles dataset with mixture components, where Danorm achieves the lowest bits (6.66). When examining the RMSE scores, Dalap benefits considerably from multiple mixture components, achieving competitive RMSE performance while maintaining the best bits scores. As we consider bits to be the most valuable metric for evaluating distributional modeling quality—since it directly measures how well the model captures the probability distribution—we suggest Dalap as the preferred alternative for discrete data modeling.

Furthermore, our other distribution function, Bitwise, performs well on highly dispersed or varied datasets in terms of bits, but exhibits significantly increased RMSE scores compared to other distribution functions. This suggests that errors in higher-order bits cause the predicted values to drift substantially, leading to large absolute errors despite reasonable probability assignments.

The Laplace, Dnormal, and Danorm functions perform similarly across most datasets, which is expected given their structural similarities in how the distributions are formulated. All three achieve reasonable performance, with Danorm showing particular strength in the mixture setting for the Bicycles dataset.

Finally, Dweib underperforms across multiple metrics, demonstrating its limitations when dealing with under- or over-dispersed data. Its performance on the Upvotes dataset is particularly poor (143.15 bits), and it fails to converge on the Migration dataset, highlighting its unsuitability for data with extreme dispersion characteristics.

When comparing against the squared error baseline (which uses a continuous relaxation), we observe that the continuous approach achieves the best RMSE in three out of four datasets. This suggests that when RMSE is the primary concern and a discrete distribution is not strictly required, continuous relaxations are most likely to provide the best performance, although exceptions exist. However, when a proper discrete distribution is needed---for example, to compute valid log-probabilities or to combine losses from discrete and continuous predictions---Dalap offers the best balance of bits and RMSE performance.

% Count data table
\begin{table*}[hbt!]
  \centering
\sisetup{detect-weight,
         group-minimum-digits = 4,
         mode=text
         }
  \caption{Test set results bicycles, migration, upvotes and maestro, best in bold}
  \begin{adjustbox}{center}
      \begin{tabular}{ l  
      	S[table-format=2.2] S[table-format=3.2]   % bicycles
      	S[table-format=2.2] S[table-format=4.2]   % upvotes
      	S[table-format=2.2] S[table-format=10.2]  % migration
      	S[table-format=1.2] S[table-format=2.2]   % maestro
      	} 
      	\hline
        ~ & \multicolumn{2}{c}{Bicycles} & \multicolumn{2}{c}{Upvotes} &  \multicolumn{2}{c}{Migration} &  \multicolumn{2}{c}{MAESTRO} \\
        ~         & {Bits}      & {RMSE}       & {Bits}      & {RMSE}        & {Bits}       & {RMSE}          & {Bits}      & {RMSE} \\
        \Xhline{1pt}
        {Dalap}            & \bfseries 6.76 & 127.98       & \bfseries 6.75 & \bfseries 118.45 & \bfseries 22.80 & 168970.89 & \bfseries 5.08 & 53.96 \\
        {Bitwise}          & 7.98        & 16148.97        & 6.85           & 8104.27       & 22.94        & 3343366400      & 5.16        & \bfseries 42.83 \\
        {Laplace}          & 6.98        & 67.56           & 7.17           & 394.50        & 66.44        & \bfseries 169328.44 & 5.42     & 47.85 \\
        {Dnormal}          & 6.89        & \bfseries 67.38 & 7.10           & 577.67        & 23.25        & 169328.44        & 5.59        & 51.12 \\
        {Dweib}            & 7.25        & 115.48          & 143.15         & 2179.24       & {na}         & {na}            & 5.81        & 65.98 \\
        {Danorm}           & 7.31        & 141.59          & 8.12           & 1786.70       & 4942.77      & 169358.13       & 5.26        & 48.87 \\
        \hline
        {Squared error}    & {na}        & \bfseries 46.51 & {na}            & 1081.69      & {na}          & \bfseries 40396.65        & {na}        & \bfseries 31.77 \\
        \hline
      \end{tabular}
  \end{adjustbox}
  \label{tab:test_res_non_mixed}
\end{table*}
% Count data table
\begin{table*}[hbt!]
  \centering
  \sisetup{detect-weight,
         group-minimum-digits = 4,
         mode=text
         }
  \caption{Test set results for mixture models on bicycles, migration, upvotes and maestro, best in bold.}
  \begin{adjustbox}{center}
      \begin{tabular}{ l 
      	c S[table-format=2.2] S[table-format=3.2]   % bicycles
      	c S[table-format=2.2] S[table-format=4.2]   % upvotes
      	c S[table-format=2.2] S[table-format=10.2]  % migration
      	c S[table-format=1.2] S[table-format=2.2]   % maestro
      	} 
      	\hline
        ~ & \multicolumn{3}{c}{Bicycles} & \multicolumn{3}{c}{Upvotes} &  \multicolumn{3}{c}{Migration} &  \multicolumn{3}{c}{MAESTRO} \\
        ~ & {K} & {Bits} & {RMSE} & {K} & {Bits} & {RMSE} & {K} & {Bits} & {RMSE} & {K} & {Bits} & {RMSE} \\
        \Xhline{1pt}
        {Dalap}   & 4 & 6.83 & 136.31          & 8 & \bfseries 6.50 & \bfseries 119.87  & 8 & \bfseries 17.73 & \bfseries 0.001   & 8 & \bfseries 4.85 & \bfseries 54.13 \\
        {Bitwise} & 8 & 7.93 & 4852.08         & 4 & 6.89 & 2538136                     & 8 & 17.96 & 3279238144                   & 8 & 5.15 & 87.99 \\
        {Laplace} & 2 & 6.79 & 66.88           & 8 & 6.50 & 293.95                      & 2 & 18.72 & 18807.51           & 8 & 4.90 & 53.53 \\
        {Dnormal} & 2 & 6.84 & \bfseries 66.13 & 8 & 6.52 & 711.04                      & 8 & 19.01 & 41321.02                     & 8 & 4.94 & 57.40 \\
        {Dweib}   & 8 & 7.14 & 110.57          & 8 & 6.51 & 544.83                      & {na} & {na} & {na}                       & 8 & 4.90 & 54.72 \\
        {Danorm}  & 8 & \bfseries 6.66 & 92.51  & 4 & 6.56 & 1020.62                 & 8 & 1908.68 & 169328.91                  & 8 & 4.85 & 55.45 \\
        \hline
      \end{tabular}
  \end{adjustbox}
  \label{tab:test_res_mixture}
\end{table*}

\subsection{PixelCNN Pixel Regression}
For image modeling tasks, we evaluate the distribution functions on MNIST, FashionMNIST, and CIFAR10 datasets. Results are presented in Tables \ref{tab:test_res_images} and \ref{tab:test_res_images_mixture} for single and mixture models respectively, and Tables \ref{tab:fid_res_images} and \ref{tab:fid_res_images_mixed} for FID scores.

We exclude Dweib and Danorm from the PixelCNN experiments due to practical limitations. Dweib exhibited numerical instability during preliminary experiments, particularly when modeling the bounded [0, 255] range required for pixel values, leading to frequent convergence failures. Danorm, while theoretically sound, requires computing a numerical approximation of the partition function by summing over a range of integers (as described in Section~\ref{section:danorm}). For image generation, this computation must be performed for every pixel in every image in the batch, causing requiring large amounts of memory. In our experiments, Danorm required over 90GB of VRAM—exceeding our available hardware capacity---making it impractical for image modeling tasks.

\subsubsection{Bits and RMSE}  
Dalap demonstrates strong performance across all image datasets. In the non-mixture setting (Table \ref{tab:test_res_images}), Dalap achieves the best bits per dimension on MNIST (0.61) and FashionMNIST (1.23), and performs competitively on CIFAR10 (3.11 bits per dimension), only marginally behind Laplace (3.09). The small difference of 0.02 bits per dimension on CIFAR10 is negligible in practice, especially considering Dalap's superior performance on the other datasets.

In the mixture setting (Table \ref{tab:test_res_images_mixture}), Dalap maintains its strong performance with 0.66 bits per dimension on MNIST, matching FashionMNIST performance at 1.23, and achieving the best result on CIFAR10 (3.0206 bits per dimension). When comparing against Dlogistic Dalap outperforms it on CIFAR10 by 0.0027 bits per dimension, and shows comparable performance on MNIST (0.66 vs 0.67). This demonstrates that Dalap can match or exceed the performance of the established discretized continuous distribution while maintaining a truly discrete formulation.

Examining RMSE scores, Dalap consistently achieves the lowest values in both single and mixture settings across all datasets. In the mixture models, Dalap achieves RMSEs of 330.48 (MNIST), 317.12 (FashionMNIST), and 510.64 (CIFAR10). This indicates that Dalap not only models the probability distribution well but also produces accurate point predictions. The combination of low bits per dimension and low RMSE suggests that Dalap effectively balances capturing the full distribution with providing reliable predictions of the expected value.

Bitwise shows significantly worse performance on image data, with bits per dimension more than double that of Dalap in most cases. This is particularly pronounced in the mixture setting, where Bitwise achieves 8.02 bits per dimension on CIFAR10 compared to Dalap's 3.02. The high RMSE values for Bitwise (e.g., 5051.66 on CIFAR10 mixture models) further confirm that representing pixels bit-by-bit introduces substantial prediction errors, likely due to the cascade effect where errors in high-order bits compound into large absolute errors.

The discretized continuous distributions (Laplace and Dnormal) show reasonable performance but generally fall short of Dalap. Laplace performs well on CIFAR10 in both settings but struggles on MNIST (24.47 bits per dimension in the non-mixture case), suggesting that simple discretization may not capture the distribution effectively for all image types. Dnormal exhibits similar patterns, with particularly poor performance on grayscale images.

\begin{table*}[hbt!]
  \centering
  \sisetup{detect-weight,
         group-minimum-digits = 4,
         mode=text
         }
  \caption{Test set results for image modeling on MNIST, FashionMNIST and CIFAR10, best in bold.}
  \begin{adjustbox}{center}
      \begin{tabular}{ l 
      	S[table-format=2.2] S[table-format=5.2]   % MNIST
      	S[table-format=1.2] S[table-format=10.2]   % FashionMNIST
      	S[table-format=1.2] S[table-format=4.2]   % CIFAR10
      	} 
      	\hline
        ~ & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{FashionMNIST} & \multicolumn{2}{c}{CIFAR10} \\
        ~ & {Bits per dim.} & {RMSE} & {Bits per dim.} & {RMSE} & {Bits per dim.} & {RMSE} \\
        \Xhline{1pt}
        {Dalap}     & \bfseries 0.61 & \bfseries 252.99   & \bfseries 1.23 & \bfseries 317.12   & 3.11 & \bfseries 479.58 \\
        {Bitwise}   & 1.63 & 535.27                       & 3.76 & 880.95                       & 5.66 & 1534.06 \\
        {Laplace}   & 24.47 & 453.39                      & 5.84 & 383.16                       & \bfseries 3.09 & 527.23 \\
        {Dnormal}   & 9.10 & 3991.58                      & 7.91 & 3710.93                      & 3.37 & 529.69 \\
        \hline
      \end{tabular}
  \end{adjustbox}
  \label{tab:test_res_images}
\end{table*}

\begin{table*}[hbt!]
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
  \sisetup{detect-weight,
          group-minimum-digits = 4,
          mode=text
          }
  \caption{Test set results for mixture models with a K of 10 on MNIST, FashionMNIST and CIFAR10, best in bold.}
  \begin{adjustbox}{center}
      \begin{tabular}{ l 
        S[table-format=2.2] S[table-format=4.2]   % MNIST
        S[table-format=1.2] S[table-format=4.2]   % FashionMNIST
        S[table-format=1.2] S[table-format=4.2]   % CIFAR10
        } 
        \hline
        ~ & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{FashionMNIST} & \multicolumn{2}{c}{CIFAR10} \\
        ~ & {Bits per dim.} & {RMSE} & {Bits per dim.} & {RMSE} & {Bits per dim.} & {RMSE} \\
        \Xhline{1pt}
        {Dalap}     & \bfseries 0.66 & \bfseries 330.48 & \bfseries 1.23 & \bfseries 317.12 & \bfseries 3.02 & \bfseries 510.64 \\
        {Bitwise}   & 2.71 & 6753.35                    & 4.98 & 5698.50   & 8.02 & 5051.66 \\
        {Laplace}   & 3.43 & 1085.34                    & 2.20 & 3538.91   & 3.05 & 515.21 \\
        {Dnormal}   & 3.97 & 1643.09                    & 3.09 & 1110.96   & 3.07 & 515.73 \\
        {Dlogistic} & 0.67 & 401.76                     & 1.37 & 554.59      & 3.02 & 554.59 \\
        \hline
      \end{tabular}
  \end{adjustbox}
  \label{tab:test_res_images_mixture}
\end{table*}

\subsubsection{Fréchet Inception Distance}  
In the FID scores of generated samples (Tables \ref{tab:fid_res_images} and \ref{tab:fid_res_images_mixed}), we observe nuanced performance patterns that depend on both the dataset and the specific generation task.

In the non-mixture setting (Table \ref{tab:fid_res_images}), Dalap achieves the best seeded sampling performance on MNIST (16.12) and FashionMNIST (52.08), demonstrating its ability to generate high-quality samples when conditioned on partial input. For CIFAR10, Laplace achieves the best seeded sampling score (45.74), closely followed by Dalap (49.76). For random sampling, Dalap excels on MNIST (33.19), while Laplace performs best on CIFAR10 (115.11). Interestingly, Bitwise achieves the best reconstruction FID scores in the non-mixture setting across all datasets (65.50, 105.50, 119.5), suggesting that its representation may preserve fine-grained details well during reconstruction despite its poor performance in likelihood modeling.

The mixture setting (Table \ref{tab:fid_res_images_mixed}) reveals a different pattern. Dlogistic dominates reconstruction tasks across all datasets, achieving FID scores of 42.00 (MNIST), 37.75 (FashionMNIST), and 26.50 (CIFAR10). This superior reconstruction performance likely stems from the smoothness properties of the underlying continuous distribution, which may better capture the perceptual structure of images. However, for sampling tasks, the performance is more balanced. Dalap achieves the best random sampling scores on MNIST (64.75) and FashionMNIST (171.59), while Dlogistic performs best on CIFAR10 (101.71). For seeded sampling, Dlogistic excels on MNIST (18.80), Dalap on FashionMNIST (62.56), and CIFAR10 shows competitive performance across multiple distributions with Laplace (41.12), Dnormal (42.12), and Dalap (44.73) all achieving similar scores.

These results indicate that the choice of distribution for image generation depends on the specific application requirements. Dlogistic offers superior reconstruction quality, making it preferable for tasks like image compression or autoencoding where faithful reproduction is most important. However, Dalap demonstrates competitive or superior performance for sampling tasks, particularly on grayscale datasets (MNIST, FashionMNIST), while maintaining better likelihood scores (bits per dimension) as shown in Tables \ref{tab:test_res_images} and \ref{tab:test_res_images_mixture}. The consistently strong performance of Dalap across both likelihood estimation and generative quality metrics suggests it is a robust choice for pixel-level modeling tasks where both probabilistic modeling and sample quality matter.

Bitwise, despite its competitive reconstruction FID in the non-mixture setting, shows poor performance in mixture models and across all sampling tasks, reinforcing our earlier observation that bit-level errors cascade into perceptually significant artifacts. Dnormal exhibits mixed performance, occasionally achieving competitive scores (e.g., 42.12 for CIFAR10 seeded sampling in a mixture setting) but lacking consistency across tasks and datasets.

\begin{table*}[hbt!]
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
  \sisetup{
    detect-weight,
    group-minimum-digits = 4,
    mode=text
  }
  \caption{FID scores on test set for image modeling on MNIST, FashionMNIST and CIFAR10, best in bold.}
  \begin{adjustbox}{center}
      \begin{tabular}{ l 
        S[table-format=2.2] S[table-format=4.2] S[table-format=4.2] % MNIST (3 cols)
        S[table-format=2.2] S[table-format=4.2] S[table-format=4.2] % FashionMNIST (3 cols)
        S[table-format=2.2] S[table-format=4.2] S[table-format=4.2] % CIFAR10 (3 cols)
      } 
      	\hline
        ~ & \multicolumn{3}{c}{MNIST} & \multicolumn{3}{c}{FashionMNIST} & \multicolumn{3}{c}{CIFAR10} \\
        ~ & {Reconstruction} & {\makecell{Seeded \\Samples}} & {\makecell{Random \\Samples}} & {Reconstruction} & {\makecell{Seeded \\Samples}} & {\makecell{Random \\Samples}} & {Reconstruction} & {\makecell{Seeded \\Samples}} & {\makecell{Random \\Samples}} \\
        \Xhline{1pt}
        {Dalap}   & 230.00 & \bfseries 16.12  & \bfseries 33.19  &  236.00 & \bfseries 52.08  & \bfseries 153.67 &   308.00 & 49.76  & 145.79 \\
        {Bitwise} & \bfseries 65.50  & 55.91  & 90.28  &            \bfseries 105.50 & 144.59 & 298.84 &   \bfseries 119.5  & 210.99 & 290.48 \\
        {Laplace} & 145.00 & 108.78 & 106.51 &                      258.00 & 101.54 & 225.68 &   308.00 & \bfseries 45.74  & \bfseries 115.11 \\
        {Dnormal} & 438.00 & 273.79 & 353.82 &                      372.00 & 267.92 & 380.73 &   294.00 & 66.90  & 146.14 \\
        \hline
      \end{tabular}
  \end{adjustbox}
  \label{tab:fid_res_images}
\end{table*}

\begin{table*}[hbt!]
  \centering
  \small
  \setlength{\tabcolsep}{3pt}
  \sisetup{
    detect-weight,
    group-minimum-digits = 4,
    mode=text
  }
  \caption{FID scores for mixture models with a K of 10 on test set for image modeling on MNIST, FashionMNIST and CIFAR10, best in bold.}
  \begin{adjustbox}{center}
      \begin{tabular}{ l 
        S[table-format=2.2] S[table-format=4.2] S[table-format=4.2] % MNIST (3 cols)
        S[table-format=2.2] S[table-format=4.2] S[table-format=4.2] % FashionMNIST (3 cols)
        S[table-format=2.2] S[table-format=4.2] S[table-format=4.2] % CIFAR10 (3 cols)
      } 
      	\hline
        ~ & \multicolumn{3}{c}{MNIST} & \multicolumn{3}{c}{FashionMNIST} & \multicolumn{3}{c}{CIFAR10} \\
        ~ & {Reconstruction} & {\makecell{Seeded \\Samples}} & {\makecell{Random \\Samples}} & {Reconstruction} & {\makecell{Seeded \\Samples}} & {\makecell{Random \\Samples}} & {Reconstruction} & {\makecell{Seeded \\Samples}} & {\makecell{Random \\Samples}} \\
        \Xhline{1pt}
        {Dalap}     & 232.00 & 54.30  & \bfseries 64.75  &            258.00 & \bfseries 62.56  & \bfseries 171.59  &  306.00 & 44.73  & 125.91 \\
        {Bitwise}   & 316.00 & 286.83 & 372.20 &                      296.00 & 275.49 & 397.46                      &  394.00 & 264.30 & 406.53 \\
        {Laplace}   & 232.00 & 155.40 & 186.08 &                      304.00 & 206.83 & 389.42                      &  306.00 & 41.12  & 138.01 \\
        {Dnormal}   & 249.00 & 180.32 & 217.04 &                      306.00 & 145.61 & 218.43                      &  308.00 & 42.12  & 189.47 \\
        {Dlogistic} & \bfseries 42.00  & \bfseries 18.80  & 90.28  &  \bfseries 37.75  & 69.18  & 200.33            &  \bfseries 26.50  & \bfseries 40.58  & \bfseries 101.71 \\
        \hline 
      \end{tabular}
  \end{adjustbox}
  \label{tab:fid_res_images_mixed}
\end{table*}

Overall, these experiments demonstrate that Dalap offers state-of-the-art performance for discrete pixel prediction, matching or exceeding the established discretized logistic mixture approach in likelihood estimation while maintaining competitive generative quality, particularly for sampling tasks. The visual samples in Figures \ref{fig:seeded_samples} and \ref{fig:random_samples} confirm that the quantitative improvements in bits per dimension translate to perceptually high-quality generated images.

\subsubsection{Generated Samples}
To qualitatively assess the generative capabilities of the mixture models, we present visual samples in Figures \ref{fig:seeded_samples} and \ref{fig:random_samples}. These figures show results from the mixture models (K=10) which provide the best results.

% SEEDED SAMPLING FIGURE
\begin{figure*}[t]
  \centering
  % MNIST row
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/dalap/MNIST/seeded_epoch_000_16.png}
    \caption{MNIST Dalap}
    \label{fig:seeded_mnist_dalap}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/dlogistic/MNIST/seeded_epoch_000_16.png}
    \caption{MNIST Dlogistic}
    \label{fig:seeded_mnist_dlogistic}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/bitwise/MNIST/seeded_epoch_000_16.png}
    \caption{MNIST Bitwise}
    \label{fig:seeded_mnist_bitwise}
  \end{subfigure}
  
  \vspace{0.3cm}
  
  % FashionMNIST row
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/dalap/Fashion/seeded_epoch_000_16.png}
    \caption{FashionMNIST Dalap}
    \label{fig:seeded_fashion_dalap}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/dlogistic/Fashion/seeded_epoch_000_16.png}
    \caption{FashionMNIST Dlogistic}
    \label{fig:seeded_fashion_dlogistic}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/bitwise/Fashion/seeded_epoch_000_16.png}
    \caption{FashionMNIST Bitwise}
    \label{fig:seeded_fashion_bitwise}
  \end{subfigure}
  
  \vspace{0.3cm}
  
  % CIFAR10 row
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/dalap/CIFAR10/seeded_epoch_000_16.png}
    \caption{CIFAR10 Dalap}
    \label{fig:seeded_cifar_dalap}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/dlogistic/CIFAR10/seeded_epoch_000_16.png}
    \caption{CIFAR10 Dlogistic}
    \label{fig:seeded_cifar_dlogistic}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{images/bitwise/CIFAR10/seeded_epoch_000_16.png}
    \caption{CIFAR10 Bitwise}
    \label{fig:seeded_cifar_bitwise}
  \end{subfigure}
  
  \caption{Seeded sampling results from mixture models (K=10). The top portion of each image is provided as conditioning, and the model generates the remainder. Dalap produces high-quality completions across all datasets, with performance comparable to Dlogistic (PixelCNN++) with lower log-likelihood. Bitwise exhibits visible artifacts, particularly on CIFAR10, consistent with its poor quantitative performance.}
  \label{fig:seeded_samples}
\end{figure*}

% RANDOM SAMPLING FIGURE
\begin{figure*}[t]
  \centering
  % MNIST row
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/dalap/MNIST/random_epoch_000.png}
    \caption{MNIST Dalap}
    \label{fig:random_mnist_dalap}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/dlogistic/MNIST/random_epoch_000.png}
    \caption{MNIST Dlogistic}
    \label{fig:random_mnist_dlogistic}
  \end{subfigure}
  \hfill
  
  \vspace{0.3cm}
  
  % FashionMNIST row
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/dalap/Fashion/random_epoch_000.png}
    \caption{FashionMNIST Dalap}
    \label{fig:random_fashion_dalap}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/dlogistic/Fashion/random_epoch_000.png}
    \caption{FashionMNIST Dlogistic}
    \label{fig:random_fashion_dlogistic}
  \end{subfigure}
  \hfill
  \vspace{0.3cm}
  
  % CIFAR10 row
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/dalap/CIFAR10/random_epoch_000.png}
    \caption{CIFAR10 Dalap}
    \label{fig:random_cifar_dalap}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{images/dlogistic/CIFAR10/random_epoch_000.png}
    \caption{CIFAR10 Dlogistic}
    \label{fig:random_cifar_dlogistic}
  \end{subfigure}
  \hfill
  
  \caption{Random (unconditional) sampling results from mixture models (K=10). All images are generated from scratch without any conditioning. Dalap generates diverse, realistic samples across all datasets, achieving the best FID scores on MNIST (64.75) and FashionMNIST (171.59). Bitwise produces visibly corrupted samples, particularly evident in the color channels of CIFAR10, demonstrating the failure mode of bit-level representation for image generation.}
  \label{fig:random_samples}
\end{figure*}

\FloatBarrier


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

